Reasoning or Pattern Exploitation? Mechanistic Insights from RL-Trained Language Models

Large language models (LLMs) are increasingly described as acquiring "reasoning" skills after reinforcement learning with verifiable rewards. However, whether these gains reflect genuine reasoning or more superficial adaptations remains underexplored. In this work, we probe LLMs trained in a finite and exhaustively analyzable logical domain, namely Tic-Tac-Toe, and trace how internal representations evolve across reinforcement learning (RL) with Group Relative Policy Optimization (GRPO). Quantitatively, RL yields high accuracy and robustness across prompt variations, suggesting the emergence of game reasoning. Mechanistic interpretability, however, paints a different picture: features extracted with sparse autoencoders (SAEs) reveal that models primarily adapt to rely more heavily on information already explicit in the prompt, such as whose turn it is, game progression and board occupancy. In comparison, high-level concepts like board symmetries and strategic forks remain weakly represented, raising concerns that reasoning benchmarks overestimate model abilities. This suggests that RL-driven "reasoning" may conflate task-specific adaptations to input information with reasoning ability. We provide, for the first time: (i) a systematic interpretability pipeline tracing representation dynamics across RL training in small-scale LLMs; (ii) an extension of SAE-based feature discovery to hypothesis-driven testing in a finite logical domain; and (iii) an interpretability-based demonstration that RL post-training neither adds nor removes concept information but reorganizes which features dominate the representation, with causal interventions locating the decision downstream of it, in the late-layer state.

==> revisions/tables/format_vs_grpo.tex <==
\begin{tabular}{lcccc}
\toprule
 & \multicolumn{2}{c}{Off-the-shelf + structured gen.} & \multicolumn{2}{c}{GRPO}\\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
Model & Legal & Best & Legal & Best\\
\midrule
Qwen2.5-1.5B & 11.7 & 8.0 & 100.0 & 75.6\\
Qwen2.5-0.5B & 26.8 & 0.4 & 56.3 & 42.1\\
Llama3.2-1B & 16.2 & 8.0 & 36.4 & 27.3\\
\bottomrule
\end{tabular}


==> revisions/tables/sae/cluster_stats_layer_strip.tex <==
\begin{tabular}{lccccccccccc}
\toprule
Hypothesis & L4 & L8 & \textbf{L12} & L13 & L14 & L15 & L16 & L17 & L18 & L20 & L24 \\
\midrule
H1 turn identity & 270 & 140 & \textbf{316} & 114 & 269 & 188 & 95 & 2208 & 5379 & 1508 & 5484\\
H2 game progression & 1151 & 594 & \textbf{2330} & 412 & 1278 & 287 & 358 & 747 & 284 & 114 & 400\\
H3 strategic situation & 123 & 68 & \textbf{194} & 63 & 136 & 53 & 69 & 187 & 86 & 32 & 126\\
H4 symmetry class & 4 & 3 & \textbf{12} & 3 & 5 & 2 & 2 & 13 & 42 & 7 & 23\\
H7 line-purity template & 28 & 24 & \textbf{39} & 27 & 33 & 36 & 23 & 22 & 13 & 17 & 12\\
\bottomrule
\end{tabular}


==> revisions/tables/sae/cluster_stats_trajectory.tex <==
\begin{tabular}{lccc}
\toprule
Hypothesis & Base & Mid & Final \\
\midrule
H1 turn identity & 5285 & 366 & 316\\
H2 game progression & 274 & 1686 & 2330\\
H3 strategic situation & 82 & 181 & 194\\
H4 symmetry class & 26 & 9 & 12\\
H7 line-purity template & 11 & 38 & 39\\
\bottomrule
\end{tabular}

